Accelerated carrier invoice factoring using predictive freight transport events

Invoice factoring is an invoice financing process where business organizations sell their invoices to banks or financial institutions at a discount to gain faster access to the invoice amount. In global trade, ocean and land carriers exercise invoice factoring to gain quick access to the money they get paid for the shipment of consignments by shippers. Shippers typically clear the invoice payment within 60-90 days of goods getting delivered. In order to get early access to capital, carriers initiate invoice factoring after the completion of goods delivery to the shipper. In this work, we provide an approach to enable accelerated carrier invoice factoring even before the delivery of goods. Carrier invoice value for a given shipment depends on the actual values of shipment tracking events. We predict the carrier invoice value at different freight transport milestone events as the goods transportation progresses from supplier to shipper using smart contracts on a blockchain network that is operated by the global trade logistics participants. The prediction at a given stage is based on past shipment tracking events and predicted future shipment tracking events. Accurate prediction of invoice value for ongoing shipment enables the carrier organization to initiate invoice factoring on the trade finance network before the completion of goods delivery to the shipper. Further, based on the past accuracy of prediction models, the financial institutions may choose to release the invoice amount in installments at different freight transportation milestone events.

==> sections/delete.tex <==
TO DO:

Expand system design to include the details on the additional outputs generated by AI service, and their visibility level setting.
Include the WORKFLOW diagram in the implement details

Include details on the acronyms used in the implementation like PO, DA, PA.

Include the reference on the milestone events.


Convey that the proposed idea is applicable to invoice discounting as well.


# Problem description should convey how we are computing the AI powered/enabled Predictive invoices and the use-case around invoice factoring.

# Capture that both the TL and WT are network built on the Hyperledger Fabric \cite{HLF}. And mention that a separate channel can be created for the payment settlment between Bank and carrier, this includes the data fetched from the TL network as part of the accelated invoice factoring. Similarly, a different channel can be created on WT containing the bank and shipper to process the payment from shipper to the bank in open accounts. Similarly, mention that there can be a separate channel for the reward settlment between the carrier and the AI Service on WT network. Moreover, the bank also might communicate with the AI service in the process of the calculating the accuracy of the estimates on the future milestone events by AI service.
======================

E-invoice is generated on blockchain via smart contracts, and both shippers and carriers can verify any generated e-invoice. Since both the shippers and carriers have access to the service contract agreements and the container tracking events and the smart contract logic used in the computation of the charges/invoices. The blockchain peers continue to monitor the shipment and perform estimates of the milestones of the shipment. The AI model considers the actual container events, and the estimated events from different blockchain peers in the process of estimating future container events. This process also helps for further learning / training the AI model.


AI Model Training:
AI model training is carried out with the help of historical shipment data. In particular, the data included actual container tracking events, and the estimated container tracking events. The model can be an RNN model.

Container tracking is done using the TradeLens (TradeLens is a blockchain based platform for interaction among the global trade supply chain participants like shippers, carriers, suppliers, logistic service providers, port authorities, government agencies, etc.). You can include the reference https://www.tradelens.com/ .

Where is the AI model located and running.  If it is updated / retrained based on additional shipment information, how is this performed and what entity retrains the model? 
If the owner of the AI model is one of the supply chain participants (e.g., supplier or shipper or carrier or factoring company), then the AI model can be run on the peer owned by the participant who is owner of the AI serve. If the owner of the AI service is not one of these existing participants, then the AI service owner can own a peer which will be part of the blockchain network. Alternatively, the AI service can be external to blockchain, and one of the participants (carrier is the most suitable) submits the estimated events on behalf of the AI model.

What new data is being stored in a block of the blockchain and where is the new data being stored (header, data section, metadata)? 

The new data to be stored is the estimated events computed by the AI model. They will be stored in the same way as the other container tracking events (either actual occurred container tracking events or estimated container occurrence events from other supply chain participants like ocean carriers, land carriers, drayage providers, etc.). 
The other additional new data is the e-invoices computed on blockchain by smart contracts using the AI model estimated events, already happened container tracking actual events and the service contract agreements. These e-invoices are stored on blockchain in the same way as the other e-invoices.
All this new data is stored in “data section” of the blocks.

====================

Though we talked about the carrier invoice factoring with respect to the ocean carriers, the similar technique is applicable to other forms of transportation companies like land (tucks and rail) or air carriers also.
Include few financial organizations that provide freight invoice factoring

